Modular Probabilistic Models via Algebraic Effects

Probabilistic programming languages (PPLs) allow programmers to construct statistical models and then simulate data or perform inference over them. Many PPLs restrict models to a particular instance of simulation or inference, limiting their reusability. In other PPLs, models are not readily composable. Using Haskell as the host language, we present an embedded domain specific language based on algebraic effects, where probabilistic models are modular, first-class, and reusable for both simulation and inference. We also demonstrate how simulation and inference can be expressed naturally as composable program transformations using algebraic effect handlers.

==> sec/elaborated-version/contributions.tex <==
\section{Contributions}


==> sec/elaborated-version/evaluation.tex <==
\section{Experimental Evaluation}

\subsection{Quantitative Evaluation}

\subsection{Qualitative Evaluation}


==> sec/elaborated-version/main.tex <==
\input{sec/elaborated-version/evaluation}

\input{sec/elaborated-version/related-work}


==> sec/elaborated-version/related-work.tex <==
\section{Related Work}
PPL development is a vigorous and active research field, being pertinent for a vast number of applications such as artificial intelligence, market research, and pharmaceutical statistics \cite{letham2016bayesian, racine1986bayesian, gelman2006data}. A difficulty with PPLs is that they can either tend to be too low-level to capture general-purpose descriptions of models, or so high-level that the treatment of models is extremely restrictive. In this paper, we capture models in their most general form as first-class citizens.

\subsection{Algebraic Effects for PPLs}

The abstraction of probabilistic models as effects and inference algorithms as effect handlers is a relatively new approach still being investigated by the machine learning community \cite{dippl, tolpin2016design}, and its existing literature is small. {\'S}cibior \& Kammar \cite{scibior2015effects} demonstrate in Haskell how inference algorithms can be abstracted as effect handlers to implement rejection sampling, and suggest effect handlers as a tool to combine inference algorithms using handler composition. Moore \& Gorinova \cite{moore2018effect} then propose the use of effect handlers on probabilistic programs to incorporate effects such as sample tracing and conditioning in languages Pyro \cite{pyro} and Edward2 \cite{edward2} embedded in Python.

This notion of executing probabilistic models using interpreters for inference algorithms is an already prevalent technique in PPLs, and we find this idea comparable in spirit to algebraic effects; many PPLs accomplish this by incorporating concurrency, coroutines, and continuation passing style transformations \cite{dippl, tolpin2016design, pymc3, pyro}. However, properly incorporating algebraic effects into PPLs has previously remained an unexplored area. The language which most closely resembles ours is Pyro which is, as far as we know, the only other PPL that takes direct inspiration from effect handlers:

\subsubsection{A Comparison with Pyro as a PPL with Effect Handlers}
Pyro \cite{pyro} views effect handlers as ``context managers'' that compose to record and modify the behaviour of probabilistic programs; this resembles our proposed design at a high-level and similarly allows probabilistic operations to be interpreted for both simulation and inference.

Pyro differs fundamentally from our work in that its inspiration from algebraic effects is rather light/informal: its implementation is more akin to a message-passing coroutine system where handlers are coroutines invoked multiple times during the course of the program, rather than them used to execute the actual program. Here, the handlers of a probabilistic program are ``context managers'' that are first pushed onto a ``handler stack''. The effectful operations are then normal Python functions that are able to broadcast messages to the handler stack. A probabilistic program is then executed for a \textit{single} iteration under the entire context of this stack, where encountering an effectful operation in the program will trigger a message to be propagated up through \textit{all} handlers, thereby invoking their individual side-effects; during this, handlers can interact by augmenting properties of this message.

\lbreaksmall
Our approach and one of our main novelties is the concrete, detailed implementation of PPLs using the instead stronger, more formal notion and structure of algebraic effects, in order to demonstrate their combined potential. Here, we strictly delineate between the syntax and semantics of models by representing models as pure syntax trees of probabilistic operations. Effect handlers are then mechanisms which individually iterate over the program themselves to provide semantics to the program, interacting with \textit{only} their own associated effectful operations. A novelty that extends from this approach is how we achieve interpretations of models for specific use-cases; we consider effect handlers for inference algorithms as purely syntactic transformations that compositionally inject algorithm-specific operations into the model.

Another contribution of our work is the exploration of PPLs with effects in a functional, strongly-typed setting. Pyro works in a weakly-typed, imperative paradigm where handlers relies on a system of mutable structures for mechanisms such as message passing and information storing to retain their state between different invocations. The lack of type information also means models themselves can contain side-effects, and handlers do not associate themselves with particular effect types/operations nor do they explicitly discharge effects. Moreover, models themselves frequently use handlers in a higher-order fashion; interleaving handlers with computations is a recognised issue \cite{wu2014effect} regarding the scope of effects, which can lead to unpredictable results. The combination of these factors, means that the behaviour of models and handlers can be arbitrary and not statically reliable. The inability to record and maintain the existing effects in a program further ambiguates the expected behaviour of running handlers and their correct composition, which is especially detrimental in probabilistic programs where incorrect behaviour of models is difficult to recognise.

In contrast, our setting emphasizes a distinction between syntax and semantics, making it clear to the programmer that side-effects are completely isolated to handlers; the application of our handlers must then be used in a first-order manner externally from models in order to retain this distinction. Our language is then transparent in what the permitted behaviours and interactions of these handlers are through their type definitions. Although we leave the formal semantics of our language for future work, our design provides a necessary foundation for reasoning equationally/theoretically about how effects interact and distribute throughout probabilistic programs, and hence about their behaviour and correctness.


\subsubsection{A Comparison with Monad Transformers as an Approach to Effects in PPLs}
A primary alternative to algebraic effects are monad transformers, seen adopted as a solution in a query-based PPL by {\'S}cibior \& Kammar \cite{mbayes}. Queries are constructed as abstract monads \lstinline{m} which must derive type classes for sampling and conditioning \cite{mbayes}. The concrete representations of these abstract monads, instantiated during model execution, express possible effects required for inference.

Here they recognised that inference algorithms can be considered to decompose into specific effects/building-blocks \cite{mbayes}, and that by abstracting these components as monadic data structures, an inference algorithm can be constructed as the composition of these using a monad transformer (MTL) approach \cite{liang1995monad}. Inference is then performed via lifting monadic operations throughout the monad stack which is viewed as applying transformations to particular layers in the stack. This can be viewed comparably with our method, in that we both consider program transformations as a series of passes in a compilation stage to take a model and augment it with new inference-specific operations. Our approaches differ primarily in how these transformations are performed; whereas we perform transformations on models as abstract syntax trees via effect handler composition, the transformations given by {\'S}cibior et al. directly execute their models via composition of monadic functions.

In terms of the high-level user interface of constructing models, in some aspects both the monad transformer library and algebraic effect approaches are similar in ease of usability and their required type-level constraints for models. Both approaches encourage specifying a minimal amount of effects for each code fragment, leading to effect constraints being propagated in a bottom-up fashion throughout the program, often without much thought for control.

However, we find the MTL approach much more complex in terms of understanding what effect an operation call corresponds to because of the necessary implicit or explicit ``lifting'' of operations: in a monad transformer stack, we implement the operations of sampling/observing as methods in a type class which each monad must implement an instance of -- these instances may confusingly defer these operation calls further up the transformer stack, implement them directly, or do both. This limits the transparency of the language mainly for the developer in terms of making it difficult to extend or implement inference algorithms. This also complicates things for the user: as there is no delineation between the semantics and syntax of models using monads in general, the model itself is immediately an effectful computation -- the user is then often required to pay attention to what the implementation of their model actually means by corresponding it to the desired inference algorithm used. One of the main goals of probabilistic programming is to separate probabilistic modelling from inference -- we find that our approach draws a more definitive line between these two notions as model syntax and semantics, and as a result, its infrastructure becomes more coherent and extensible.

Additionally there is very frequently a need for coroutine behaviour or intermediate representations of models as syntax trees during inference; monad transformers would need to include explicit monads for these effects (e.g. the \lstinline{FreeT} or \lstinline{Coroutine} monad), whereas algebraic effects inherently provide these features. This conflates the two notions of models as monadic computations and models as syntax, which can be confusing.

\subsection{Embedding Techniques for PPLs}

We have found the ability to represent models as syntax trees as a highly desirable property for model-based PPLs which algebraic effects accommodates for: this allows for a very flexible interpretation of models and probabilistic operations by inference algorithms, and being able to performing passes of transformations over these trees breaks lets us incrementally implement the semantics of inference algorithms in a fine-grained manner. Additionally, the algebraic effect approach is sufficiently minimalistic in capturing only the effects we care about as syntax.

\lbreaksmall
\citeauthor{scibior2015practical} also take approaches which can be considered similar to ours, as proof-of-concept that the monad abstraction can be used to construct probabilistic models whilst still offering good performance during inference. Their language avoids free monads as an underlying structure and instead directly encodes distributions as an intermediate free monad representation. Distributions are syntactically constructed by standard monadic composition and semantics are provided using type classes, allowing individual components to be sampled from. An important point to note is that they also embed conditional distributions as part of their representation, meaning their language is \textit{query-based}.

\lbreaksmall
Two main alternative embedding techniques which would allow one to create a delineation between model syntax and semantics are deep embeddings and tagless-final style. Deep embeddings are too heavy-duty for our needs; as is well-known, this approach tends to lead to the embedded language becoming unwieldy and overly distinct from the host language \cite{svenningsson2015combining}. Tagless-final shallow embedding \cite{kiselyov2012typed} has been used to correspond PPL syntax to type class methods, where different class instances correspond to different representations over the entire language \cite{kiselyov2016probabilistic, kiselyov2009embedded, narayanan2016probabilistic}. This is however more suited for \textit{uniformly} applying a semantic domain over the entirety of a program; this makes it difficult to perform iterations of transformations (such as interpretations to sample and observe) over models, and hence harder to achieve inference in a composable manner.

\lbreaksmall
Other PPLs which do achieve a proper model-based implementation typically require some form of special compilation stage for models. General-purpose PPLs (Turing.jl \cite{turingjl}, Gen.jl \cite{genjl}) tend to take advantage of the macro-compilation features of their host language to rewrite the syntax trees of models into executable functions. Special-purpose PPLs implement models as their own language construct, which are then compiled to entirely different languages (Stan \cite{stan}, BUGS \cite{bugs}).


\subsection{Model Environments}
Model-based languages require mechanisms for specifying observed data to models to interpret operations to sample and observes. Similar to us, Pyro also uses effect handlers to let observed values be specified to random variable names by the user providing a dictionary environment. However, this does not accommodate ``traces'' of values i.e. observable variables have only one dynamic instance throughout the execution of a model, and can not provide a static guarantee about the correct type of value provided nor whether a certain observable variable exists in a model. In other general-purpose model-based PPLs, this is typically done using global variables or function arguments \cite{tolpin2016design, dippl, kiselyov2009embedded}, macro-compilation \cite{turingjl}, Gen.jl \cite{genjl}, providing mappings between addresses and observed data \cite{genjl}, and defining default behaviour for missing function arguments \cite{turingjl}. Special-purpose PPLs allow models and observed data to be specified independently as special language constructs, where common variables are consolidated during compilation  \cite{stan, bugs}. Extensible records have not previously been seen to be adopted as a solution.


==> sec/sir-equations.tex <==
\begin{align*}
  &\text{If} \quad &\frac{dR}{dt} &= \gamma I\\
  &\text{Then this implies that $I$ must be of the form} \quad &I &= e^{\gamma t}\\
  &\text{This is because of the general rule that if} \quad &y &= e^{\gamma t}, \text{then } \frac{dy}{dt} = \gamma e^{\gamma t} = \gamma y\\
  &\text{In other words, $I$ can take no other form that would result in } &\frac{dR}{dt} &= \gamma I\\
  &\text{Therefore}&I &= e^{\gamma t}\\
  &&\frac{dR}{dt}  &= \gamma I = \gamma e^{\gamma t}\\
  &\text{If $I = e^{\gamma t}$, when $t$ is 0, $I = 1$. As $t$ increases linearly, $I$ increases exponentially.}\span\span\\
  &\text{If $I = e^{-\gamma t}$, when $t$ is 0, $I = 1$. As $t$ increases, $I$ will decrease from $1$ to $0$} \span\span&\\
  &\text{The probability $1 - e^{-\gamma t}$ means that if $\gamma$ or $t$ increases, $e^{-\gamma t}$ will go from $1$ to $0$}\span\span\\
  &\text{so the probability will become higher.}\span\span
\end{align*}
